Rapid Approximate Aggregation with Distribution-Sensitive Interval Guarantees

Aggregating data is fundamental to data analytics, data exploration, and OLAP. Approximate query processing (AQP) techniques are often used to accelerate computation of aggregates using samples, for which confidence intervals (CIs) are widely used to quantify the associated error. CIs used in practice fall into two categories: techniques that are tight but not correct, i.e., they yield tight intervals but only offer asymptotic guarantees, making them unreliable, or techniques that are correct but not tight, i.e., they offer rigorous guarantees, but are overly conservative, leading to confidence intervals that are too loose to be useful. In this paper, we develop a CI technique that is both correct and tighter than traditional approaches. Starting from conservative CIs, we identify two issues they often face: pessimistic mass allocation (PMA) and phantom outlier sensitivity (PHOS). By developing a novel range-trimming technique for eliminating PHOS and pairing it with known CI techniques without PMA, we develop a technique for computing CIs with strong guarantees that requires fewer samples for the same width. We implement our techniques underneath a sampling-optimized in-memory column store and show how to accelerate queries involving aggregates on a real dataset with speedups of up to 124x over traditional AQP-with-guarantees and more than 1000x over exact methods.

==> algofix.tex <==

\makeatletter
\renewcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2}\algocf@typo:}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax%
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else%
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi%
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\everypar={\relax}}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~##1\par}%
    \algocf@linesnumbered%
  }}%
\makeatother

==> dap-proof.tex <==

A key idea behind our distribution-aware techniques for estimating the
mean of a finite dataset rests on the principle that the empirical CDF
constructed from independent random samples from some distribution tends
to concentrate around the true CDF, an intuition that is quantified by
the DKW inequality~\cite{massart1990tight}. We need to similarly quantify
this intuition in the case that samples are taken without replacement
from a finite dataset, as a practical system must reduce cache misses and
leverage locality in storage hierarchies by sampling without
replacement via a scan along shuffled data.
It turns out that the DKW inequality holds in this case
as well; we state this fact here and defer a proof to later.
\begin{restatable}{lemma}{dkwnoreplace}
\label{lem:dkwnoreplace:dd}
For any $N > 0$, the DKW inequality applies for sampling without replacement
from a finite dataset of size $N$.
\end{restatable} 

To prove correctness of \Cref{alg:dap:dd}, we will make extensive use
of the following fact from earlier, which we state without proof:
\cdfmean*

In \Cref{lem:sufficient:dd}, we now give sufficient conditions
for correctness of the intervals returned by \Cref{alg:dap:dd}; i.e., conditions sufficient
for ensuring that returned interval $[\Li, \Ui]$ contains $\AVG(\dataset)$.
In \Cref{lem:iteration:dd}, we will then show that the input $\delta$ to the algorithm
allows us to tune the number of samples taken such that these conditions are satisfied
with arbitrarily high probability.
\begin{lemma}
\label{lem:sufficient:dd}
For any $0<\el<\ar<1$,
the following conditions are sufficient to guarantee that
$\Li \leq \AVG(\dataset)$ as computed by \Cref{alg:dap:dd} at iteration $\iter$:
\begin{enumerate}[label=(\roman*)]
	\item $\AVG(\whdslp) - \vepsl \leq \AVG(\dslp)$
	\label{cond:hsleft:dd}
	\item $\AVG(\whdsrp) - \vepsr \leq \AVG(\dsrp)$
	\label{cond:hsright:dd}
	\item $\sup |F - \ecdf| \leq \edkw$
	\label{cond:dkw:dd}
\end{enumerate}
where $F$ is the true CDF for the distribution taken by a single sample drawn uniformly randomly from $\dataset$,
$\ecdf$ is the empirical CDF corresponding $\whds$,
$\whdslp$ is set to $\whdsl$,
and $\whdsrp$ is set to $\whdsr$.
Again for any $0<\el<\ar<1$ (possibly different),
the above conditions are likewise sufficient to guarantee that
$\AVG(\dataset) \leq \Ui$ for
$\whdslp$ set to $1-\whdsre$ and $\whdsrp$ set to $1-\whdsle$.
\end{lemma}
\begin{proof}
We prove the case for $\Li$; the case for $\Ui$ is symmetric by noting that
\[ \AVG(\dataset) \leq \Ui \Longleftrightarrow 1-\Ui \leq \AVG(1-\dataset) \]
If conditions~\ref{cond:hsleft:dd} and~\ref{cond:hsright:dd} hold, then we have that
\begin{align}
\Li &=\quad \plp(\AVG(\whdsl) - \vepsl) + \prm(\AVG(\whdsr) - \vepsr) \\
	&\quad\quad\quad + (1-\plp-\prm)\AVG(\whdsmm) \nonumber \\
	&\leq\quad \plp\AVG(\dsl) + \prm\AVG(\dsr) \label{eqn:proveusingdkw:dd} \\
	&\quad\quad\quad + (1-\plp-\prm)\AVG(\whdsmm) \nonumber
\end{align}
We will show that condition~\ref{cond:dkw:dd} implies that \Cref{eqn:proveusingdkw:dd}
is a lower bound for $\AVG(\dataset)$.
To do so, will write $\AVG(\dataset)$ in terms of
$\cdfl$, $\cdfm$, and $\cdfr$ --- the CDFs resulting from the distributions taken by individual
samples from $\dsl$, $\dsm$, and $\dsr$, respectively. First, define $\ecdfp$ as
\[ \forall x \in [a, b], \ecdfp(x) \equiv \min\{\ecdf(x) + \edkw, 1\} \]
Note that
\begin{subequations}
\label{eqn:propsfromcdf:dd}
\begin{equation}
\label{eqn:lpropfromcdf:dd}
\pls = F(\el)
\end{equation}
\begin{equation}
\label{eqn:mpropfromcdf:dd}
\pms = F(\ar)-F(\el)
\end{equation}
\begin{equation}
\label{eqn:rpropfromcdf:dd}
\prs = 1-F(\ar)
\end{equation}
\begin{equation}
\label{eqn:lpropfromcdfupper:dd}
\plp = \min\{|\whdsl|/|\whds| + \edkw, 1\} = \ecdfp(\el)
\end{equation}
\begin{equation}
\label{eqn:rpropfromcdfupper:dd}
\prm = \max\{|\whdsr|/|\whds| - \edkw, 0\} = 1-\ecdfp(\ar)
\end{equation}
\end{subequations}
Then we have that
\begin{align}
&\AVG(\dataset) = 1 - \int_0^1 F(x)dx \label{step:integralmean:dd} \\
   &= \pls\left(\el - \frac{1}{\pls}\int_0^{\el}F(x)dx\right) \label{step:simplifiestoprev:dd} \\
       &\quad + \prs\left(1 - \frac{1}{\prs}\int_{\ar}^1(F(x) - \pls - \pms)dx\right) \nonumber \\
       &\quad + \pms\ar + (\ar-\el)\pls - \int_{\el}^{\ar}F(x)dx \nonumber \\
   &= \pls\left(\el - \int_0^{\el}\cdfl(x)dx\right)
    + \prs\left(1 - \int_{\ar}^1\cdfr(x)dx\right) \label{step:restrictedcdf:dd} \\
    &\quad + \pms\ar + (\ar-\el)\pls - \int_{\el}^{\ar}F(x)dx \nonumber \\
   &= \pls(\mul - \el + \ar)
    + \pms\ar
    + \prs\mur
    - \int_{\el}^{\ar}F(x)dx \label{step:integralmean2:dd} \\
   &= F(\el)(\mul - \el + \ar)
    + (F(\ar) - F(\el))\ar \label{step:propstocdfeval:dd} \\
    &\quad\quad + (1-F(\ar))\mur 
                - \int_{\el}^{\ar}F(x)dx \nonumber \\
   &\geq \inf_{\{f : \sup|f-\ecdf|\leq\edkw\}} f(\el)(\mul - \el + \ar)
    + (f(\ar) - f(\el))\ar \label{step:dkwbound:dd} \\
    &\quad\quad + (1-f(\ar))\mur
    - \int_{\el}^{\ar}f(x)dx \nonumber \\
   &= \inf_{\{f : \sup|f-\ecdf|\leq\edkw\}} f(\el)(\mul - \el)
    + f(\ar)(\ar - \mur) \nonumber \\
    &\quad\quad + \mur - \int_{\el}^{\ar}f(x)dx \nonumber \\
   &= \ecdfp(\el)(\mul - \el)
    + \ecdfp(\ar)(\ar - \mur) \label{step:maximizenegativequants:dd} \\
    &\quad\quad + \mur - \int_{\el}^{\ar}\ecdfp(x)dx \nonumber \\
   &= \plp(\el)(\mul - \el)
    + (\plp + \pmh)(\ar - \mur) \label{step:cdfevaltoprops:dd} \\
    &\quad\quad + \mur - \int_{\el}^{\ar}\ecdfp(x)dx \nonumber \\
   &= \plp\mul
    + \prm\mur
    + \pmh\ar - \int_{\el}^{\ar}(\ecdfp(x) - \plp)dx \nonumber \\
   &= \plp\mul 
    + \prm\mur \nonumber \\
    &\quad\quad + \pmh\left(\ar - \frac{1}{\pmh}\int_{\el}^{\ar}(\ecdfp(x) - \plp\right)dx \nonumber \\
   &= \plp\mul
    + \pmh\AVG(\whdsmm)
    + \prm\mur \label{discardfromcdfupper:dd} \\
   &= \plp\mul
    + (1-\plp-\prm)\AVG(\whdsmm)
    + \prm\mur \nonumber \\
   &= (\ref{eqn:proveusingdkw:dd}) \nonumber
\end{align}
Each of the numbered steps is justified as follows: \\
(\ref{step:integralmean:dd}) follows from \Cref{lem:cdfmean:dd}; \\
(\ref{step:simplifiestoprev:dd}) can be verified to simplify to (\ref{step:integralmean:dd}) via direct manipulation; \\
(\ref{step:restrictedcdf:dd}) follows by noting that CDFs for distributions with
truncated support can be constructed from non-truncated CDF by subtracting
off the proportion of the original distribution lying to the left of the truncated support,
followed by scaling so that the truncated CDF evaluates to $1$ at the rightmost value of the
truncated support; \smacke{Might need another lemma if this step is too hard.} \\
(\ref{step:integralmean2:dd}) follows from another application of \Cref{lem:cdfmean:dd}; \\
(\ref{step:propstocdfeval:dd}) follows from \Cref{eqn:lpropfromcdf:dd,eqn:mpropfromcdf:dd,eqn:rpropfromcdf:dd}; \\ %
(\ref{step:dkwbound:dd}) follows from condition~\ref{cond:dkw:dd}: if $\sup|F-\ecdf| \leq \edkw$, then $F$
lies in a $\edkw$-neighborhood of $\ecdf$, so the value of $f$ that gives the smallest value of
(\ref{step:dkwbound:dd}) in this neighborhood must necessarily be a lower bound for (\ref{step:propstocdfeval:dd}); \\
(\ref{step:maximizenegativequants:dd}) follows by noting that the quantities $\mul-\el$, $r-\mur$, and $-f(x)$
are all negative, so we want to choose $f$ to maximize $f(x)$ everywhere in $[\el, \ar]$, subject to
the constraint that $\sup|f-F|\leq\edkw$, which is precisely attained at $f\equiv\ecdfp$; \\
(\ref{step:cdfevaltoprops:dd}) follows from
\Cref{eqn:lpropfromcdfupper:dd,eqn:rpropfromcdfupper:dd}; \\
(\ref{discardfromcdfupper:dd}) follows from noting that $\ecdfp$ is the CDF corresponding to
the distribution taken by a random sample from $\whdsmm$, and then applying \Cref{lem:cdfmean:dd}.
Thus, conditions~\ref{cond:hsleft:dd} -- \ref{cond:dkw:dd} are sufficient to ensure that $\Li \leq \AVG(\dataset)$.
\end{proof}

\begin{lemma}
\label{lem:iteration:dd}
For any $\iter$, the probability that \Cref{alg:dap:dd} computes $[\Li, \Ui]$
such that $\AVG(\dataset)\notin[\Li, \Ui]$
is less than $\frac{6\delta}{\pi^2\iter^2}$.
\end{lemma}
\begin{proof}
\smacke{Fill me in. None of Serfling and DKW failure events ensure
conditions of \Cref{lem:sufficient:dd} are met; probability of any of these
failure events is at most sum of various $\delta$s by union bound.}
\end{proof}



\begin{theorem}
\label{thm:correctness:dd}
The probability that \Cref{alg:dap:dd} returns a value further than
$\veps$ away from $\AVG(\dataset)$ is at most $\delta$.
\end{theorem}
\begin{proof}
At each round $\iter$, the probability that
$\AVG(\dataset) < \Li$ or $\AVG(\dataset) > \Ui$
is at most $6\delta / \pi^2\iter^2$, by \Cref{lem:iteration:dd}.
Union bounding over rounds, the probability that the returned value is
bad is therefore at most
\[ \sum_{\iter\geq1}\frac{6\delta}{\pi^2\iter^2} = \delta \cdot \frac{6}{\pi^2}\sum_{\iter\geq1}\iter^{-2} = \delta \]
where we used the identity $\sum_{\iter\geq1}\iter^{-2} = \frac{\pi^2}{6}$.
\end{proof}

\dkwnoreplace*
\begin{proof}
Sketch: following the original paper from Wald and Wolfowitz
on confidence limits for CDFs~\cite{wald1939confidence},
it suffices to consider the CDF for mass distributed uniformly
at each integer $1, 2, \ldots, N$. For each without-replacement
sample size $m$ and each deviation $\veps$, we would like to be
able to claim that
\[ \Parg{\sup|F_N - \ecdf_{N,m}| \geq \veps} < \Parg{\sup|F_{N'} - \ecdf_{N',m}| \geq \veps} \]
for every $N' > N$ --- that is, in some sense, the CDF becomes monotonically ``harder''
to estimate as we increase the dataset size. Unfortunately, this turns out to
not be the case, but in fact the claim follows if we merely prove the weaker condition
that
\[ \Parg{\sup|F_N - \ecdf_{N,m}| \geq \veps} < \Parg{\sup|F_{N'} - \ecdf_{N',m}| \geq \veps} \]
for {\em infinitely many} $N' > N$, implying that, as $N' \rightarrow \infty$,
the resulting probability to which $\Parg{\sup|F_{N'} - \ecdf_{N',m}|}$ converges
(necessarily bounded by the probability computed in the DKW inequality)
is an upper bound for the corresponding probability at every
finite $N'$, from which the claim would follow.

We show this via construction: namely, we show that, for every $N$, $m$, and $\veps$,
\[ \Parg{\sup|F_N - \ecdf_{N,m}| \geq \veps} < \Parg{\sup|F_{2N} - \ecdf_{2N,m}| \geq \veps} \]
That is, the CDF becomes monotonically harder to estimate each time we double the dataset size.
To show this, we consider two cases. Case 1: if point $2i-1$ is sampled, then point $2i$ is not
sampled, and vice versa for every $i=1,\ldots,N$. Conditioned on this event, the probability that
$\sup|F_{2N} - \ecdf_{2N,m}| \geq \veps$ at least the (unconditioned) probability that
$\sup|F_N - \ecdf_{N,m}| \geq \veps$, since samples at odd indices can only increase the deviation,
and samples at even indices cannot decrease it. Case 2: there is at least one $i$ for which points
at both indices $2i-1$ and $2i$ are sampled. Each such point is conceptually similar to
reducing $m$ by 1 in the original dataset of size $N$, but randomly weighting one of the samples
by 2 instead of 1. It can be shown that each time this is done, the probability that
$\sup|F_N - \ecdf_{N,m}| \geq \veps$ increases.
\end{proof}


==> dap.tex <==
\begin{algorithm}[h]
\caption{The \dap algorithm}\label{alg:dap:dd}
\algrenewcomment[1]{\texttt{/*} #1 \texttt{*/} \\}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\SetKwBlock{Repeat}{Repeat}{}
\SetKwProg{myfunc}{function}{}{}
\SetKwFunction{lbound}{conf\_lbound}
\SetKwFunction{dkw}{dkw}
\SetKwFunction{serfling}{serfling}
{\scriptsize
\Input{Dataset $\dataset$ of values in $[0,1]$, parameters $\veps$ and $\delta$, boundaries $\el^{\csub}, \ar^{\csub}, \el^{\cadd}, \ar^{\cadd}$}
\Output{Estimate for $\AVG(\dataset)$ and error bounds at most $\veps$ in length}
\nonl\ \\
\myfunc{\dkw{$\delta\cpp,\ m\cp$}\textnormal{\ ~\cite{dvoretzky1956asymptotic,massart1990tight}}}{
\Comment{two-sided $\delta\cpp$-level confidence bound for $\sup|F-\ecdf|$
after taking $m\cp$ samples (with or without replacement)}
\Return{$\sqrt{0.5/m\cp \cdot \log{\frac{2}{\delta\cpp}}}$}\;
}
\myfunc{\serfling{$\delta\cpp,\ m\cp,\ N\cp$}\textnormal{\ ~\cite{bardenet2015concentration,serfling1974probability}}}{
\Comment{one-sided $\delta\cpp$-level confidence bound for mean of $m\cp$ without-replacement samples
taken from $N\cp$ points in $[0,1]$}
\Return{$\sqrt{0.5/m\cp \cdot \left(1 - \frac{m\cp-1}{N\cp}\right) \cdot \log{\frac{1}{\delta\cpp}}}$}\;
}
\myfunc{\lbound{$\delta\cp,\whds\cp,\el,\ar$}}{
\label{dap:line:lboundfunc-start}
\label{dap:line:lboundfunc:dd}
$\ecdf\cp \gets \text{ empirical CDF based on $\whds\cp$}$\;
$\edkw \gets$ \dkw{$\delta\cpp\myeq\delta\cp/2,\ m\cp\myeq|\whds\cp|$}\;
	$\whdslp \gets \{x \in \whds\cp : x < \el\}$\;
\label{lbound:line:compute-lb-start}
	$\whdsrp \gets \{x \in \whds\cp : x \geq \ar\}$\;
	$\whdsmp \gets \{x \in \whds\cp : \el \leq x < \ar\}$\;
	\label{lbound:line:compute-edkw}
	$\plp \gets \min\{|\whdslp|/|\whds\cp| + \edkw, 1\}$\;
	$\prp \gets \min\{|\whdsrp|/|\whds\cp| + \edkw, 1\}$\;
	$\prm \gets \max\{|\whdsrp|/|\whds\cp| - \edkw, 0\}$\;
	$\vepsl \gets \el\cdot$ \serfling{$\delta\cpp\myeq\delta\cp/4,\ m\cp\myeq|\whdslp|,\ N\cp\myeq\plp |\dataset|$}\;
	$\vepsr \gets (1-\ar)\cdot$ \serfling{$\delta\cpp\myeq\delta\cp/4,\ m\cp\myeq|\whdsrp|,\ N\cp\myeq\prp |\dataset|$}\;
	\label{lbound:line:compute-vepsl}
	$\whdsmmp \gets \{x \in \whdsmp : \ecdf\cp(x) \leq 1-\edkw\}$\;
	\Return{$\plp(\AVG(\whdslp) - \vepsl) 
	+ \prm(\AVG(\whdsrp) - \vepsr)
	+ (1-\plp-\prm)\AVG(\whdsmmp)$}\;
\label{lbound:line:compute-lb-end}
\label{dap:line:lboundfunc-end}
}
\nonl\ \\
\label{dap:line:init:dd}
$\whds\gets\emptyset$\;
\For{$\iter\gets 1,2,\ldots,\infty$}{
\label{dap:line:loop:dd}
	\smacke{$\el^{\csub}, \ar^{\csub}, \el^{\cadd}, \ar^{\cadd}$ should be allowed to change between iterations}\;
	$\whds \gets \whds \cup \{\text{additional without-replacement samples from $\dataset$}\}$\;
	$L_{\iter} \gets $\lbound{$6\delta/\pi^2\iter^2,\whds,\el^{\csub},\ar^{\csub}$}\;
\label{dap:line:computevepsils:dd}	
	$U_{\iter} \gets 1-$\lbound{$6\delta/\pi^2\iter^2,1-\whds,\el^{\cadd},\ar^{\cadd}$}\;
\label{dap:line:computevepsirs:dd}	
	\If{$U_{\iter} - L_{\iter} \leq \veps$ \textbf{or} $|\whds| = |\dataset|$}{
\label{dap:line:test:dd}
		\textbf{break}\;
	}
}
\Return{$\AVG(\whds), [L_{\iter} - \AVG(\whds), U_{\iter} - \AVG(\whds)]$}
}
\end{algorithm}


==> fishbounder.tex <==

\begin{algorithm}[t]
\caption{Fishman error bounder~\protect\cite{fishman1991confidence}}\label{alg:fishbounder:dd}
\algrenewcomment[1]{\texttt{/*} #1 \texttt{*/} \\}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\SetKwBlock{Repeat}{Repeat}{}
\SetKwProg{myfunc}{function}{}{}
\SetKwFunction{init}{init\_state}
\SetKwFunction{update}{update\_state}
\SetKwFunction{lbound}{Lbound}
\SetKwFunction{rbound}{Rbound}
{\scriptsize
\nonl\ \\
\myfunc{\init{}}{
\Return{\upshape{\texttt{\big\{$c$: $0$, $\xbar$: $0$\big\}}}}\;
}
\nonl\ \\
\myfunc{\update{$S, v$}}{
$c' \gets S.c + 1$\;
$\xbar' \gets S.\xbar + (v - S.\xbar) / c'$\;
\Return{\upshape{\texttt{\big\{$c$: $c'$, $\xbar$: $\xbar'$\}}}}\;
}
\nonl\ \\
\myfunc{\lbound{$S, a, b, N, \delta$}}{
\uIf{$S.\xbar = a$}{
\Return{\upshape{$a$}}\;
}\uElse{
$\xbar' \gets (S.\xbar - a)/(b-a)$\;
Find $t$ such that $0<t<\xbar'$ and $\KL{\xbar'-t}{t} = \frac{\log{(1/\delta)}}{S.c}$\;
\Return{\upshape{$a + t\cdot(b-a)$}}\;
}
}
\nonl\ \\
\myfunc{\rbound{$S, a, b, N, \delta$}}{
$S.\xbar \gets (a+b) - S.\xbar$\;
\Return{\upshape{$(a+b) - \lbound(S, a, b, N, \delta)$}}\;
}
}
\end{algorithm}


==> macros.tex <==

\makeatletter
\newcommand*{\declarecommand}{%
  \@star@or@long\declare@command
}
\newcommand*{\declare@command}[1]{%
  \provide@command{#1}{}%
  \renew@command{#1}%
}
\makeatother

\newcommand{\na}{\textsf{N/A}}
\makeatletter
\newcommand*{\phd}{%
    \@ifnextchar{.}%
        {Ph.D}%
        {Ph.D.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\prof}{%
    \@ifnextchar{.}%
        {Prof}%
        {Prof.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\dr}{%
    \@ifnextchar{.}%
        {Dr}%
        {Dr.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\etal}{%
    \@ifnextchar{.}%
        {et al}%
        {et al.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\resp}{%
    \@ifnextchar{.}%
        {resp}%
        {resp.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\whp}{%
    \@ifnextchar{.}%
        {w.h.p}%
        {w.h.p.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\iid}{%
    \@ifnextchar{.}%
        {i.i.d}%
        {i.i.d.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\lhs}{%
    \@ifnextchar{.}%
        {L.H.S}%
        {L.H.S.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\rhs}{%
    \@ifnextchar{.}%
        {R.H.S}%
        {R.H.S.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\wrt}{%
    \@ifnextchar{.}%
        {w.r.t}%
        {w.r.t.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\sthat}{%
    \@ifnextchar{.}%
        {s.t}%
        {s.t.\@\xspace}%
}
\makeatother

\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\numof}{num.\@\xspace}

\def\densesection#1{\vspace{-3pt}\section{#1}\vspace{-3pt}}

\newenvironment{densecenter}{%
  \setlength\topsep{0pt}
  \setlength\parskip{0pt}
  \begin{center}
}{%
  \end{center}
}

\mdfdefinestyle{MyFrame}{%
  linecolor=gray,
  outerlinewidth=0.25pt,
  roundcorner=3pt,
  innertopmargin=\baselineskip,
  innerbottommargin=\baselineskip,
  innerrightmargin=10pt,
  innerleftmargin=10pt,
  backgroundcolor=white
}

\newenvironment{dingenum}{
  \begin{enumerate}[label=\protect\bcircle{\arabic*}]
}{\end{enumerate}}

\newenvironment{denselist}{
    \begin{list}{\small{$\bullet$}}%
    {\setlength{\itemsep}{0ex} \setlength{\topsep}{0ex}
    \setlength{\parsep}{0pt} \setlength{\itemindent}{0pt}
    \setlength{\leftmargin}{1.5em}
    \setlength{\partopsep}{0pt}}}%
    {\end{list}}

\newenvironment{denseenum}{
  \begin{enumerate}[
  wide=0pt,
  widest=99,
  leftmargin=\parindent,
  labelsep=*,
  topsep=2pt,
  partopsep=0pt,
  parsep=0pt,
  itemsep=1pt,
  ]
}{\end{enumerate}}

\newenvironment{denseding}{
  \begin{enumerate}[
  wide=0pt,
  widest=33, %
  leftmargin=\parindent,
  labelsep=*,
  topsep=2pt,
  partopsep=0pt,
  parsep=0pt,
  itemsep=1pt,
  label=\protect\bcircle{\arabic*}
  ]
}{\end{enumerate}}

\newcommand{\topic}[1]{\vspace{-2.5pt}\smallskip \smallskip \noindent{\bf #1.}}
\newcommand{\stitle}[1]{\vspace{0.5em}\noindent\textbf{#1}}
\newcommand{\emtitle}[1]{\vspace{0.3em}\noindent{\em #1}}
\newcommand{\frameme}[1]{
\thesissub{\noindent\fbox{
  \parbox{0.95\linewidth}{
    \noindent #1
    }
  }}{\begin{mdframed}#1\end{mdframed}}
}

\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\definecolor{persiangreen}{rgb}{0.0, 0.65, 0.58}
\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{M}[1]{>{\arraybackslash}m{#1}}
\newcolumntype{$}{>{\global\let\currentrowstyle\relax}}
\newcolumntype{^}{>{\currentrowstyle}}
\newcolumntype{!}{<{\gdef\nonheader{1}}}
\newcommand{\rowstyle}[1]{\gdef\currentrowstyle{#1}%
  #1\ignorespaces
}
\makeatletter
\newcolumntype{S}[1]{>{\arraybackslash\@ifundefined{nonheader}{}{#1}}c}
\makeatother
\newcommand{\undefnonheader}{\global\let\nonheader\relax}

\NewEnviron{curlymatrix}{%
  \LEFTRIGHT\lcbrace\rcbrace{\,\begin{matrix}\BODY\end{matrix}\,}%
}
\makeatletter
\NewEnviron{curlycases}{%
  \def\arraystretch{1.2}%
  \LEFTRIGHT\lcbrace.{%
    \,\array{@{}l@{\quad}l@{}}\BODY\endarray\,
  }%
}
\makeatother

\newenvironment{algo}{%
  \renewenvironment{algocf}[1][h]{}{}%
  \algorithm
}{%
  \endalgorithm
}

\makeatletter
\newcommand{\nosemic}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\dosemic}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\pushline}{\Indp}%
\newcommand{\popline}{\Indm\dosemic}%
\let\oldnl\nl%
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}%
\makeatother

\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\bcircle}[1]{\ding{\number\numexpr 201 + #1 \relax}}
\newcommand{\qtext}[1]{\quad\text{#1}\quad} 
\newcommand\mbb[1]{\mathbb{#1}}
\def\mc#1{\mathcal{#1}}
\def\mrm#1{\mathrm{#1}}
\def\reals{\mathbb{R}} %
\def\integers{\mathbb{Z}} %
\def\rationals{\mathbb{Q}} %
\def\naturals{\mathbb{N}} %
\def\complex{\mathbb{C}} %
\def\bigo#1{\mathcal{O}\left(#1\right)} %
\renewcommand{\exp}[1]{\operatorname{exp}\left(#1\right)} %
\def\indic#1{\mbb{I}\left\{{#1}\right\}} %
\providecommand{\argmax}{\mathop\mathrm{arg max}} %
\providecommand{\argmin}{\mathop\mathrm{arg min}}
\providecommand{\arccos}{\mathop\mathrm{arccos}}
\providecommand{\dom}{\mathop\mathrm{dom}} %
\providecommand{\range}{\mathop\mathrm{range}} %
\providecommand{\diag}{\mathop\mathrm{diag}}
\providecommand{\tr}{\mathop\mathrm{tr}}
\providecommand{\abs}{\mathop\mathrm{abs}}
\providecommand{\card}{\mathop\mathrm{card}}
\providecommand{\sign}{\mathop\mathrm{sign}}
\def\rank#1{\mathrm{rank}({#1})}
\def\E{\mathbb{E}} %
\def\Earg#1{\E\left[{#1}\right]}
\def\Esubarg#1#2{\E_{#1}\left[{#2}\right]}
\def\P{\mathbb{P}} %
\def\Parg#1{\P\left({#1}\right)}
\def\Psubarg#1#2{\P_{#1}\left[{#2}\right]}
\def\Cov{\mrm{Cov}} %
\def\Var{\mrm{Var}} %
\def\Covarg#1{\Cov\left[{#1}\right]}
\def\Covsubarg#1#2{\Cov_{#1}\left[{#2}\right]}
\newcommand{\family}{\mathcal{P}} %
\newcommand{\iidsim}{
  \mathrel{\overset{iid}{\scalebox{1}{$\sim$}}}
}
\newcommand\mean[1]{\overline{#1}}
\def\Gsn{\mathcal{N}}
\def\Ber{\textnormal{Ber}}
\def\Bin{\textnormal{Bin}}
\def\Unif{\textnormal{Unif}}
\def\Mult{\textnormal{Mult}}
\def\NegMult{\textnormal{NegMult}}
\def\Dir{\textnormal{Dir}}
\def\Bet{\textnormal{Beta}}
\def\Poi{\textnormal{Poi}}
\def\HypGeo{\textnormal{HypGeo}}
\def\GEM{\textnormal{GEM}}
\def\BP{\textnormal{BP}}
\def\DP{\textnormal{DP}}
\def\BeP{\textnormal{BeP}}
\def\IG{\textnormal{IG}}

\declaretheoremstyle[
notefont=\normalfont, notebraces={[}{]},
bodyfont=\normalfont\itshape,
headformat=\NAME~\NUMBER\NOTE
]{brackets}
\ifthesis
\declaretheorem[numberwithin=chapter,style=brackets]{definition}
\declaretheorem[numberwithin=chapter]{theorem}
\declaretheorem[numberwithin=chapter]{lemma}
\declaretheorem[numberwithin=chapter]{hypothesis}
\declaretheorem[numberwithin=chapter]{corollary}
\declaretheorem[numberwithin=chapter]{example}
\declaretheorem[numberwithin=chapter]{guarantee}
\declaretheorem[numberwithin=chapter]{constraint}
\declaretheorem[numberwithin=chapter]{problem}
\else
\declaretheorem[style=brackets]{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{guarantee}{Guarantee}
\newtheorem{constraint}{Constraint}
\newtheorem{problem}{\textbf{Problem}}
\fi

\crefname{guarantee}{Guarantee}{Guarantees}
\crefname{problem}{Problem}{Problems}
\crefname{example}{Example}{Examples}
\crefname{constraint}{Constraint}{Constraints}

\newcommand\SUM{\textsf{SUM}\xspace}
\newcommand\COUNT{\textsf{COUNT}\xspace}
\newcommand\AVG{\textsf{AVG}\xspace}
\newcommand\VAR{\textsf{VAR}\xspace}
\newcommand\MIN{\textsf{MIN}\xspace}
\newcommand\MAX{\textsf{MAX}\xspace}
\newcommand\AGG{\textsf{AGG}\xspace}
\newcommand\groupby{\textsf{GROUP BY}\xspace}
\newcommand\code[1]{{\texttt{{\upshape#1}}}}
\newcommand\spacecode[1]{\,\,\texttt{{\upshape#1}}}
\newcommand\codespace[1]{\texttt{{\upshape#1}}\,\,}
\newcommand\spacecodespace[1]{\,\,\texttt{{\upshape#1}}\,\,}


\newcommand{\veps}{\varepsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\fst}{^{(1)}}
\newcommand{\snd}{^{(2)}}
\newcommand{\nth}{^{(n)}}
\newcommand{\inv}{^{-1}}
\newcommand{\ith}{^{(i)}}
\newcommand{\jth}{^{(j)}}
\newcommand{\kth}{^{(k)}}
\newcommand{\lth}{^{(l)}}
\newcommand{\tth}{^{(t)}}
\newcommand{\pskip}{\ \\ \ \\}
\def\supp#1{^{(#1)}}
\def\subp#1{_{(#1)}}
\def\norm#1{||#1||}
\def\KL#1#2{\text{KL}(#1||#2)}

\newcommand{\gcal}{\mathcal{G}\xspace}
\newcommand{\ee}{\mathcal{E}\xspace}

\newcommand{\cc}{\mathcal{C}\xspace}
\newcommand{\rr}{\mathcal{R}\xspace}
\newcommand{\hh}{\mathcal{H}\xspace}
\newcommand{\pp}{\mathcal{P}\xspace}

\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{\mathbf{1}}

\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\plus}{\scalebox{.65}{+\hspace{-2pt}}}
\newcommand{\minus}{\scalebox{.6}{$-$}}

\newcommand{\zv}{{\sf zenvisage}\xspace}
\newcommand{\ntail}{{\sf NeedleTail}\xspace}
\newcommand{\needletail}{\ntail}
\newcommand{\helix}{{\sf Helix}\xspace}
\newcommand{\fm}{{\sf FastMatch}\xspace}
\newcommand{\ff}{{\sf FastFrame}\xspace}
\newcommand{\fv}{{\sf FastFrame}\xspace}
\newcommand{\vs}{{\sf HistSim}\xspace}
\newcommand{\hsim}{\vs}
\newcommand{\vsim}{\vs}
\newcommand{\vizsim}{\vs}
\newcommand{\histsim}{\vs}
\newcommand{\dhub}{{\sc DataHub}\xspace}

\newcommand{\br}{\ \\ \texttt{*************************************************************************}\\}

\renewcommand{\emptyset}{\varnothing}
\renewcommand{\mod}[1]{(\mathrm{mod}\;{#1})}

\DeclareMathOperator{\Tr}{Tr}

\def\supregistered{\textsuperscript{\tiny\textregistered}\xspace}
\def\blah{\red{blah}\xspace}

